Optimal endorsement for network-wide distributed blockchains

Blockchains offer trust and immutability in non-trusted environments, but most are not fast enough for latency-sensitive applications. Hyperledger Fabric (HF) is a common enterprise-level platform that is being offered as Blockchain-as-a-Service (BaaS) by cloud providers. In HF, every new transaction requires a preliminary endorsement by multiple mutually untrusted parties called organizations, which contributes to the delay in storing the transaction in the blockchain. The endorsement policy is specific to each application and defines the required approvals by the endorser peers (EPs) of the involved organizations. In this paper, given an input endorsement policy, we studied the optimal choice to distribute the endorsement requests to the proper EPs. We proposed the OPEN algorithm, devised to minimize the latency due to both network delays and the processing times at the EPs. By extensive simulations, we showed that OPEN can reduce the endorsement latency up to 70% compared to the state-of-the-art solution and approximated well the introduced optimal policies while offering a negligible implementation overhead compared to them.

==> Sec8_ThechnicalDraft.tex <==
%!TEX root = main.tex

\begin{figure}[!h]
    \centering
    \includegraphics[width=4cm]{Figures/optimal endorsement2.pdf}
    \caption{Queuing model. Policy is $1$-out-of-$R$, with $R \leq Q$ queues/servers.}
    \label{figure:QueuingModel}
\end{figure}


\section{Assumptions}
\begin{itemize}
\item Poisson arrivals for transactions
\item uniform random choice of $R$ queues for each transaction
\item no network delays
\end{itemize}

\section{Endorsement delays}
Utilization factor for each server/queue:
\begin{equation}
U=\dfrac{\lambda RC}{Q\mu}\leq 1
\end{equation}
Thus, to be sustainable, the arrival rate must satisfy:
\begin{equation}
\lambda\leq \dfrac{Q\mu}{RC}
\end{equation}


\subsection{Policy 1-out-of-$R$ }

%In a M/M/1 the waiting time (queueing + service} $W$ is exponentially distributed with rate 
%$(\mu-\lambda')$ where $\lambda'$ is the actual arrival rate.

It can be shown (Paolo's note pg.~30) that the average endorsement latency for the policy 1-out-of-$R$ can be computed as follows:
\begin{equation}
E[L]=\dfrac{1}{R\mu-\dfrac{\lambda CR^2}{Q}}\qquad
R\in[1,\ldots,Q]
\end{equation}

Let $\hat{R}$ be the optimal value of $R$ that minimizes $E[L]$. It holds:
\begin{equation}\label{eq:1}
\hat{R}_{A,k1}=\dfrac{\mu Q}{2\lambda C}
\end{equation}

\subsection{Policy 2-out-of-$R$}
It can be shown (Paolo's note pg.~49) that the average endorsement latency for the policy 2-out-of-$R$ can be computed as follows:
\begin{equation}\label{eq:2}
E[L]=\dfrac{1}{\mu-\dfrac{\lambda CR}{Q}}\left(\dfrac{1}{R}+\dfrac{1}{R-1}\right)\qquad
R\in[2,\ldots,Q]
\end{equation}
The optimal value of $\hat{R}$ can be computed analytically.

\begin{equation}\label{eq:r21}
\begin{split}
\hat{R}_{A,k2} =& \dfrac{1}{12 \lambda C}(F_1 +\\ 
& \dfrac{4 \mu^2 Q^2 - 4 \mu \lambda C Q + \lambda^2 C^2}{F_1} +\\ 
&  2 \mu Q + 5 \lambda C)
\end{split}
\end{equation}

Where:

\begin{equation}\label{eq:f11}
\begin{split}
F_1 &= [8 \mu^3 Q^3 - 12 \mu^2 \lambda C Q^2 +  114 \mu \lambda^2 C^2 Q -\\ 
& 55 \lambda^3 C^3 +12 \lambda C (12 \mu^4 Q^4 - 24 \mu^3 \lambda C Q^3 +\\ 
& 99 \mu^2 \lambda^2 C^2 Q^2 - 87 \mu \lambda^3 C^3 Q + 21 \lambda^4 C^4)^{1/2}]^{1/3} 
\end{split}
\end{equation}


\section{Experiments}

To guarantee sustainable arrivals, i.e., $U\leq 1$, {\em for any $R$}, i.e., also in the case $R=Q$, it must hold:
\begin{equation}\label{eq:7}
\lambda\leq \dfrac{\mu}{C}
\end{equation}

Now we fix:
\begin{equation}\label{eq:lambda}
\lambda=\gamma\dfrac{\mu}{C}
\end{equation}
with $\gamma\in(0,1]$  being the load factor.

Now run the simulations for any $R\in[1,Q]$ and plot the endorsement delay in the function of $R$, for different values of load factor $\gamma$.
\subsection{Policy 1-out-of-$R$}

By combining~\eqref{eq:1} and~\eqref{eq:lambda}, we have:
\begin{equation}\label{eq:r1}
\hat{R}_{N,k1}=\dfrac{Q}{2\gamma}
\end{equation}

\begin{figure}[!tb]
	\centering
%	\begin{subfigure}{0.48\columnwidth}
%        \centering
%        \includegraphics[width=1\linewidth]{Figures/K1C8Q(1 to 32)-optimal_R graph.pdf}
%        \caption{Optimal R for $C=8$, $Q=(1$ to $32)$ and $k=1$}
%        % \label{figure:exp-topo}
%	\end{subfigure}\hfill
%	\begin{subfigure}{.48\columnwidth}
        \centering
        \includegraphics[width=8cm]{Figures/K1Q(1 to 32)-optimal_R graph[cliped].pdf}
        % \caption{Optimal R for $C=8$, $Q=(1$ to $32)$ and $k=1$}
        \caption{Optimal R for $Q=(1$ to $32)$ and $k=1$}
        % \label{figure:remote-controller-based}
%	\end{subfigure}
% 	\caption{Topologies employed in the experimental testbed.	}
\end{figure}


In practice the optimal value $\hat{R}$ will be chosen as the nearest integer to $\hat{R}$, clipped to the range $[1,Q]$:
\begin{equation}
% \hat{R}=\min\left\{Q,\left[\hat{R}_{N,k1}\right]\right\}
\hat{R}=\min\bigg\{Q, \left\lfloor{\hat{R}_{N,k1}}\right\rfloor\bigg\}
\end{equation}

\subsection{Policy 2-out-of-$R$}

The optimal value $\hat{R}$ will be chosen as to minimize ~\eqref{eq:2}, which by exploiting ~\eqref{eq:lambda}, we have:

\begin{equation}\label{eq:r22}
\begin{split}
\hat{R}_{N,k2} =& \dfrac{1}{12 \gamma}(F_2 +\\ 
& \dfrac{4 Q^2 - 4 \gamma Q + \gamma^2}{F_2} +\\ 
& 2 Q + 5 \gamma)
\end{split}
\end{equation}

Where:

\begin{equation}\label{eq:f12}
\begin{split}
F_2 &= (8 Q^3 - 12 \gamma Q^2 + 114 \gamma^2 Q -\\ 
& 55 \gamma^3 + 12 \gamma(12 Q^4 - 24 \gamma Q^3 +\\ 
& 99 \gamma^2 Q^2 - 87 \gamma^3 Q + 21 \gamma^4)^{1/2})^{1/3} 
\end{split}
\end{equation}


% \begin{figure}[!h]
% \centering
% \includegraphics[width=12cm]{Figures/K2C10Q(2 to 32)-optimal_R graph.pdf}
% \caption{Optimal R for $C=10$, $Q=(2$ to $32)$ and $k=2$}
% \end{figure}

\begin{figure}[!tb]
	\centering
%	\begin{subfigure}{0.48\columnwidth}
%        \centering
%        \includegraphics[width=1\linewidth]{Figures/K2C8Q(2 to 32)-optimal_R graph.pdf}
%        \caption{Optimal R for $C=8$, $Q=(2$ to $32)$ and $k=2$}
%        % \label{figure:exp-topo}
%	\end{subfigure}\hfill
%	\begin{subfigure}{.48\columnwidth}
        \includegraphics[width=8cm]{Figures/K2Q(2 to 32)-optimal_R graph[cliped].pdf}
        % \caption{Optimal R(clipped)  for $C=8$, $Q=(2$ to $32)$ and $k=2$}
        \caption{Optimal R(clipped) for $Q=(2$ to $32)$ and $k=2$}
        % \label{figure:remote-controller-based}
%	\end{subfigure}
% 	\caption{Topologies employed in the experimental testbed.	}
\end{figure}

In practice the optimal value $\hat{R}$ will be chosen as the nearest integer to $\hat{R}$, clipped to the range $[1,Q]$:
\begin{equation}
\hat{R}=\min\bigg\{Q,\left \lfloor{\hat{R}_{N,k2}}\right\rfloor\bigg\}
\end{equation}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=12cm]{Figures/K2C10Q(2 to 32)-optimal_R graph[cliped].pdf}
% \caption{Optimal R(clipped)  for $C=10$, $Q=(2$ to $32)$ and $k=2$}
% \end{figure}


\begin{figure}[!h]
\centering
\includegraphics[width=8cm]{Figures/Q(2 to 32)-optimal_R graph(k2-k1).pdf}
% \caption{Difference of optimal R for $k=1$ and $k=2$, $C=8$, $Q=(2$ to $32)$}
\caption{Difference of optimal R for $k=1$ and $k=2$, $Q=(2$ to $32)$}
\end{figure}


\begin{figure}[!h]
\centering
\includegraphics[width=8cm]{Figures/endorser.png}
\caption{Model applied for $Q=8$ and $k=1$}
\end{figure}
% \paolo{We should report also the simulation results. Just for $C=1$ since it is the same}
\begin{figure}[!h]
\centering
\includegraphics[width=8cm]{Figures/endorser-k2.png}
% \caption{Model applied for $C=Q=8$ and $k=2$}
\caption{Model applied for $Q=8$ and $k=2$}
\end{figure}


% Anytime a client wants to send a transaction to the blockchain network, it needs a proper proposal for the transaction. The proper proposal contains the simulation results of the transaction on the initial values(current world states), the related outcomes(next world state values), and signatures from the entities responsible for doing these simulations which are named endorsers. A logical expression between the organizations defines the needed endorsements for the proposal to be accepted in the next steps which are called "Endorsement policy". the equation made of AND, OR, and $k-ot-of-N$ operators on the organization  will define which endorsers    

\clearpage
\section{Algorithm}

% Any endorsement policy for a blockchain system with $N$ organizations can be converted to the form of $k$-out-of-$M_1$ statements where the statements might be a single organization, the conjunction(AND) or the disjunction(OR) of different organizations or even other sta, the client can benefit the \texttt{Optimizer} process to reduce the endorsement phase delay. 
% Knowing that the form $k$-out-of-$M_1$ can be mapped always to disjunction(OR) of all possible conjunction between $k$ or more choices, we can convert this simplified form to the extended form of OR(AND($S_1$), AND($S_2$),..., AND($S_l$)) where each AND($S_i$) in the extended form is one of the conjunctions between $k$ or more choices out of $M_1$ choices.
% Doing this, we will have a $1$-out-of-$M_2$ policy at the end, where $M_2$ is the total number of the conjunctions that can be made from selecting $k$ or more out of $M_1$. 


\subsection{Endorsement policy expression}

In Hyperledger Fabric the endorsement policy is defined based on a syntax that allows the operators AND, OR, and $k$-OutOf, applied to a set of organizations, and nested expressions~\cite{hfend}. 
In particular, the operator $k$-OutOf($E$) returns true whenever at least $k$ expressions within set $E$ are satisfied.
Despite the complexity of the policy expression, the following holds:
\begin{prop}\label{ref:p1}
Any endorsement policy obtained by combining arbitrarily AND, OR, OutOf operators  is equivalent to the policy 
\begin{equation}\label{eq:or}
\text{OR}(S_1,S_2,...)
\end{equation}
 where each of $S_i$ is either a single organization or the conjunction(AND) of different organizations.
\end{prop}
\begin{proof}
In the case of expressions based on only AND and OR operators, thanks to the distribution principle in logic expressions,  we can transform the original expression in the target form~\eqref{eq:or}. In the case of $k$-OutOf$(e_1,e_2,\ldots, e_m)$ operator, where $e_i$ is a single expression,  by definition this holds:
\[
k-\text{OutOf}(e_1,e_2,\ldots, e_m)=\text{OR}(\{\text{AND}(E)\}_{E\in\Omega})
\]  
being $\Omega$ the set of all combinations of $k$ expressions from the set of $m$. Note that $|\Omega|=\binom{m}{k}$.
As an example, 
\[
\begin{split}
&\text{2-OutOf}(e_1,e_2,e_3,e_4) =\\
&\text{OR}(\text{AND}(e_1,e_2),\text{AND}(e_1,e_3),\text{AND}(e_1,e_4),\\
&\text{AND}(e_2,e_3),\text{AND}(e_2,e_4),\text{AND}(e_3,e_4))\\ 
\end{split}
\]
Now since any expression with OutOf operator is equivalent to one with only AND and OR, by following the previous reasoning, such expression can be reduced to the target expression~\eqref{eq:or}. 
\end{proof}

The result of Property~\ref{ref:p1} allows investigating only one particular form of endorsement expression, independently from the complexity of the original expression.


%Any endorsement policy for the Hyperledger Fabric with $N$ organizations can be converted to the eventual form of ``OR($S_1$,$S_2$,...,$S_i$,...,$S_l$)" where each of $S_i$ might be a single organization or the conjunction(AND) of different organizations. Also any $k$-of-$M$ policy, defined as 
%% if you end up with a policy similar to 2-out-of-$M$ 
%%where the $M$ statements are
%a policy  OR($O_1$, $O_2$ , AND($O_3,O_4$)), where $O_i$ is organization $i$, becomes 
%% (i.e., $A_3A_4$ is equivalent to AND($A_3$, $A_4$)), then we can rewrite the policy as 1-out-of-$M_1$ while the $M_1$ is \{$A_1A_2$, $A_1A_3A_4$, $A_2A_3A_4$\}, which is equivalent to 
%"OR($A_1A_2$, $A_1A_3A_4$, AND($A_2A_3A_4$). Also a policy with an AND as the outermost logic can be expressed as the OR between the "false" logic and itself(i.e., "OR(false,AND(...))"). From now, we call each of the $S_i$ inside the last extended form of the policy as an statement. It is worth noting that the reason behind interest in using the "OR" policy is that it is equivalent to need for a response with the minimum delay out of all the requests.
%


The policy defined at the organization level must be mapped into a policy defined at the peer level since the \en requests are sent from the clients directly to the peers. 
Each organization can be constituted by one or more endorsement peers. Getting the endorsement from a specific organization requires receiving it from {\em any} of its endorsement peers, which is equivalent to the policy $1$-OutOf$(p_1,p_2,\ldots)$, where $p_i$ are the peers within the organization. Revisiting Property~\ref{ref:p1} applied at the policy expression at a peer level, we can claim:
\begin{prop}\label{p2}
Any \en policy defined at organization level can be mapped into an \en policy defined at peer level as follows:
\begin{equation}\label{eq:o2}
\text{OR}(S_1,S_2,...)
\end{equation}
 where each of $S_i$ is either a single peer or the conjunction(AND) of different peers.
\end{prop}


\subsection{Endorsement Optimization}

The goal of the algorithm is to minimize the endorsement response delay by selecting some proper endorsers. The algorithm receives as input the list of all the peers $\mathcal P$, the endorsement policy in the form~\eqref{eq:o2}, a threshold for the acceptable minimum sample size, and a sampling period to set the proper rate for probe endorsements. 
%Let $X_p$ be the random variable defined with the empirical distribution of the \en latencys experienced for peer $p$ and evaluated based on both the \en requests and the probes.
As an output, the algorithm returns a set $\mathcal P_e\subseteq \mathcal P$ of peers for sending the endorsement requests.
 
The main idea of the proposed optimization procedure is the following. For the sake of the explanation, let us assume to have just one peer per organization and to know the distribution of the \en latency for each peer. We also assume to have a simple policy expression with OR of different peers. 

Each transaction is numbered sequentially with a sequence number, which is local to each client.
We denote by $\text{TX}^{(n)}$ be the transaction with sequence number $n$. Anytime a response is received by a peer, the corresponding response delay is updated.
Let $X^{(n)}=[X_p^{(n)}]_{p\in \mathcal P}$ be the response delay vector, with $X_p^{(n)}$ be the response delay of endorser peer $p$ observed for $\text{TX}^{(n)}$ and $Y^{(k)}=[Y_p^{(k)}]_{p\in \mathcal P,k=1,2}$ be the approximated response delay vectors of the last two response delay of endorser peer $p$ observed for $\text{TX}^{(k)}$. The elements in the vectors $X^{(n)}$ and $Y^{(1)}$ are initialized to $0$. Observe that $X^{k)}$ can be divided into 3 parts: (1) the delays corresponding to the peers that were selected as the endorser for the previous transaction and the endorsement reply has been already received, (2)
% denoted as $A$ 
the delays corresponding to the peers that were selected as the endorser for the previous transaction but the endorsement reply is not received yet, (3) 
% denoted as $B$
the delays corresponding to the peers that were not selected as endorsers for the previous transaction. Thus, if $X^{(k)}_p=0$, it means that the response delay from peer $p$ for the $\text{TX}^{(k)}$ is {\em undefined}, either because $\text{TX}^{(k)}$ did not send any endorsement request to peer $p$, or because the corresponding response has not arrived yet, due to processing and network delays. 
Finally, let $\mathcal X=\{X^{(k)}\}_{k=1,\ldots,n}$ be the complete history of past response delays up to current transaction $n$ and $\mathcal Y=\{Y^{(k)}\}_{k=1,2}$ be the approximated history of the last two response delays. 

%Let $P$ be the set of peers where to send the \en requests, given a transaction request. 

%The algorithm considers now all the other peers and evaluate if it is worth adding each of them to the set of peer try to consider an organization with the minimum expected value of the \en latency delays and checks if by adding another organization out of the remaining ones, whether it is capable to reduce the average of the minimum. This is done with the help of the Cumulative distribution function(CDF) of the minimum, where Optimizer1 calculates the expected value of the minimum delay samples among the selected organizations. After finding the best couple, Optimizer1 will repeat this procedure for finding the best third organization to be added to the previously found best couple. It will repeat this procedure until the theoretical enhancement of adding another organization is less than a selected threshold. At last, based on a specific rate, Optimizer1 will select one extra organization from the remaining organizations of the policy to be used as the prob request.

Based on our previous assumption of having only one peer in each organization, every time we select a different peer, it is equivalent to selecting a different organization. Similar to what was explained before, the response delays are used for updating the two previously mentioned data structures. Anytime an endorsement response is received, the \texttt{UpdateDelay} will extract the $p$ as the endorser peer number, the $m$ as the sequence number of the endorsement request, and will update the $X^{(m)}_p$ with the calculated response delay~(lines \ref{lst:line:1_00} to \ref{lst:line:1_03}). Now, if the sequence number of the endorsement request is for one of the two recent requests, it will update the corresponding temporary place for the delays of the two recent requests(i.e., $Y^{(n-m)}_p$)~(lines \ref{lst:line:1_04} and \ref{lst:line:1_05}). 

The \texttt{Optimizer} will receive the policy in the mentioned format, a list of the peers related to the policy, the list of endorsement peers used during the previous endorsement request, the transaction sequence number, the probe sampling period, a set of all the past endorsement response delays for all the peers, and a set of modified endorsement response delays for the last two recent transactions' endorsement requests~(line \ref{lst:line:1}). Now, as the representatives of the response delays for the new transaction, the two vectors $X^{(n)}$ and $Y^{(1)}$ will be initialized to $0$ with the size of all peers~(lines \ref{lst:line:1_1} to \ref{lst:line:1_3}). Then, if this is the first transaction~(line \ref{lst:line:2}), then the \texttt{Optimizer} will select all the peers as the members of the endorsers set and will return it~(lines \ref{lst:line:3} to \ref{lst:line:4}). Otherwise, the \texttt{Optimizer} will call the \texttt{SelectEndorsers} function to receive an optimized selection of the endorser peers~(line \ref{lst:line:5}). We proposed (2) variants for this function that we will explain in the next sections. To keep fresher the \en latency samples, We periodically sample the \en latencys of all the \ed peer as follows. The algorithm will send a probe(i.e., an extra endorsement request) to one of the peers that are not part of the currently selected endorsers set by the \texttt{SelectEndorsers} function. The rate of the \texttt{Probe} is controlled by the probe sampling period parameter and the transaction sequence number~(lines \ref{lst:line:6} to \ref{lst:line:10}). The pseudocode of \texttt{Optimizer} is provided in Fig.~\ref{alg:opt_endorse0}.  



\begin{figure}[!tb]
\scriptsize
\label{alg:opt_endorse0}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{ Input:}
\renewcommand{\algorithmicensure}{ Output:}
\Require $\mathcal M$: Endorsement policy at peer level in the format~\eqref{eq:o2}
\Require $\mathcal P$: Set of all the peers
\Require $\mathcal P_e^\text{old}$: Set of \ed peers used during the previous \en request
\Require $n$: Sequence number of the current transaction 
\Require $T$: Probe sampling period 
\Require $\mathcal X=\{X^{(k)}\}_{k=1,\ldots,n}$: Past history of response delays
\Require $\mathcal Y=\{Y^{(k)}\}_{k=1,2}$ : Modified version of the response delays for last two recent transactions respectively
% \algdef{SE}[VARIABLES]{Variables}{EndVariables}
%   {\algorithmicvariables}
%   {\algorithmicend\ \algorithmicvariables}
% \algnewcommand{\algorithmicvariables}{ global variables}}

% \Variables
%  \State $\mathcal Y=\{Y^{(k)}\}_{k=1,2}$ \label{lst:line:0_1} \Comment{Modified version of the response delays for $\text{TX}^{(n-1)} \text{ and } \text{TX}^{(n-2)}$ respectively}
% \EndVariables

\Procedure{UpdateDelay}{endorsment-response}\label{lst:line:1_00}
\State $p=$peer(endorsment-response)\label{lst:line:1_01} 
\State $m \gets$ sequence-number(endorsment-response)\label{lst:line:1_02}
\State $X^{(m)}_p=$response-delay(endorsment-response)\label{lst:line:1_03}
 \If{$m \geq n-2$}\label{lst:line:1_04}
   \State $Y^{(n-m)}_p=X^{(m)}_p$\label{lst:line:1_05}
  \EndIf
\EndProcedure

\Procedure{EndorsementOptimizer}{$\mathcal M,\mathcal P,\mathcal P_e^\text{old},n,T,\mathcal X,\mathcal Y$}\label{lst:line:1}
\For{$p \in \mathcal P$}\label{lst:line:1_1}
 \State $X^{(n)}_p = 0$\label{lst:line:1_2} \Comment{Initializing the $X^{(n)}$ response delays for $\text{TX}^{(n)}$}
 \State $Y^{(1)}_p = 0$\label{lst:line:1_3} \Comment{Initializing the $Y^{(1)}$ response delays for $\text{TX}^{(n)}$}
\EndFor
\If {$n=1$} \label{lst:line:2}\Comment{Initializing for the first transaction}
  \State $\mathcal P_e\gets \mathcal P$ \label{lst:line:3} \Comment{Select all the available peers}
   \State \Return $\mathcal P_e$ \label{lst:line:4} \Comment{Return the \ed list}
\EndIf
    \State $\mathcal P_e\gets$ {\tt SelectEndorsers}($\mathcal P,\mathcal P_e^\text{old},\mathcal X,\ldots$ )\label{lst:line:5} \Comment{Best endorsers}
    \If{($n \mod T = 0$)} \label{lst:line:6} \Comment{Check if it is the time for a probe}
      \State $p_r\gets$ random peer in $\mathcal P\setminus \mathcal P_e$ \label{lst:line:7} \Comment{Select a random peer not in $\mathcal P_e$}
      \State \Return $\mathcal P_e$, $p_r$ \label{lst:line:8} \Comment{Return final \ed list and a probe request}
    \Else \label{lst:line:9}
      \State \Return $\mathcal P_e$ \label{lst:line:10} \Comment{Return just final \ed list}
    \EndIf
\EndProcedure
 
\end{algorithmic}
\caption{Pseudocode of the \texttt{Optimizer} algorithm}\label{alg:opt_endorse0}
\end{figure}



\subsubsection{AveMinDelay(AMD)}

The \texttt{AveMinDelay(AMD)} procedure has $\epsilon_\text{thr}$ as the input parameter and returns a set of peers.
At first, the \texttt{AveMinDelay(AMD)} procedure initializes $p_\text{best}^+=-1$, as the best candidate peer that can be added to the set of current \ed peers for reducing the \en latency~(line \ref{lst1:line:2}). The algorithm then computes the average minimum \en latency based on the estimated distribution of the \en latencys of the previously used \ed peers $\mathcal P_e$. This value will be stored as the \texttt{bestDelay}. Now the algorithm iterates on the peers that are not part of $\mathcal P_e$, where at each iteration it calculates the difference of the average minimum \en latency after adding the new peer to the $\mathcal P_e$ with the \texttt{bestDelay}. If this difference is more than the $\epsilon_\text{thr}$, then the $p_\text{best}^+$ will be updated with the new peer and \texttt{bestDelay} will be replaced with the new reduced value. This procedure will be repeated for all peers to find the possible best choice and if there exists such a peer, the $\mathcal P_e$ will be updated by adding the $p_\text{best}^+$ to it~(lines \ref{lst1:line:4} to \ref{lst1:line:9}). 
To determine if adding a peer is beneficial or not, the \texttt{AveMinDelay(AMD)} will calculate the expected value of the minimum \en latency among this newly selected peer and the peers of the set $\mathcal P$ and will compare this against a threshold~(\ref{lst1:line:8}). This can be done numerically thanks to the knowledge of the distribution of the \en latencys for each peer. It is well known that, if the Cumulative distribution function(CDF) of $X_i$ is denoted by $F_{X_i}(t)$, then the CDF of the minimum among them is given by:
\begin{equation}
    P(Y \leq y)=F_Y(t)=1-\prod_{i} (1-F_{X_i}(t)) 
\end{equation}

In our case, for the set of peers(i.e., ($S_j = \mathcal P$ $\cup$ "new selected peers")), the $Y$ is the minimum of the statement($S_j$) delay samples and the $X_i$(s) are the samples of the organizations($O_i$) of that statement. So, the equation becomes:
\begin{equation}
    F_{S_j}(t)=1-\prod_{i}(1-F_{O_i}(t))
\end{equation}

Then, the expected value of the minimum can be calculated from:
\begin{equation}
\begin{split}
  E(S_j)&=\int_{0}^\infty(1-F_{S_j}(t))dt\\
  &=\int_{0}^\infty\prod_{i}(1-F_{O_i}(t))dt
\end{split}
\end{equation}

The \texttt{AveMinDelay(AMD)}, will check the opposite cases as well, where it searches to find a peer, except the possible $p_\text{best}^+$, in the main $\mathcal P_e$ such that by removing it from the new $\mathcal P_e$, the new average minimum \en latency again reduces more than $\epsilon_\text{thr}$. If this comes true, the mentioned peer will be removed from the $\mathcal P_e$ and the new $\mathcal P_e$ will be returned~(lines \ref{lst1:line:10} to \ref{lst1:line:18}).



% one best peer~(lines \ref{lst1:line:4} to \ref{lst1:line:11}) if this allows reducing the average minimum \en latency, based on the current estimated distribution of the \en latencys of all the peers.


% At each main iteration, there will be an internal sub-iteration where the algorithm searches for the best peer in this level by considering each peer outside the current set $P$ and evaluates the worthiness of the possible reduction in the \en latency due to the addition of the peer to $P$~(lines \ref{lst1:line:7} to \ref{lst1:line:10}). 

% At the end of each sub-iteration if a peer was added to the $P$, a \texttt{Continue} flag will be set to \texttt{true} to keep the main iteration loop active for the next level search of the new peer while the best-found peer will be added to $P$ as the reference for the new search.

% In the case no reduction is possible or the reduction is less than the mentioned threshold, as the \texttt{Continue} flag remains \texttt{false}, the main iteration will ends and $P$ is returned to the \texttt{Optimizer} algorithm. The pseoudocode of \texttt{SelectEndorsers-AveMinDelay(AMD} is provided in Fig.~\ref{alg:opt_endorse1}.

% In each level of adding a new peer, this calculation should be repeated for each peer that is not inside $P$~(line \ref{lst1:line:10}). If the new expected delay is less than the previous best case and the improvement is above the desired threshold~(line \ref{lst1:line:11}), then the new peer is selected as the best additive to $P$~(line \ref{lst1:line:12}). The new $P$ will be considered as the new starting list of endorsers~(line \ref{lst1:line:14}), where the algorithm as the next level will repeat the procedure of finding a new worthy peer. For avoiding the redundant useless search, if in an iteration over the remaining peers the conditions in~(line \ref{lst1:line:11}) do not hold for any of those peers, the "Continue" flag will remain false and the iteration will be stopped. In this step, the \texttt{SelectEndorsers-AveMinDelay(AMD} will check the counter related to the number of transactions received after the last \texttt{Probe} endorsement, and if it is equal to the \texttt{Probe} regulation rate, a new random peer from the remaining peers will be selected and added to $P$, then the counter value will be reset to zero~(lines \ref{lst1:line:15} to \ref{lst1:line:18}). At last, $P$ and the new counter value will be returned as the output of the \texttt{SelectEndorsers-AveMinDelay(AMD}.



\begin{figure}[!tb]
\scriptsize
\label{alg:opt_endorse1}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{ Input:}
\renewcommand{\algorithmicensure}{ Output:}
\Require $\mathcal P$: Set of \ed peers 
\Require $\mathcal P_e$: Candidate set of \ed peers 
\Require $\epsilon_\text{thr}$: Delay threshold [s]
\Require $\mathcal X=\{X_p\}_{p\in \mathcal P}$: Response delays for all the peers with their empirical distributions
\Procedure{SelectEndorsers-AMD}{$\mathcal P,\mathcal P_e,\mathcal X,\epsilon_\text{thr}$}\label{lst1:line:1}
\State $p_\text{best}^+=-1$ \label{lst1:line:2}\Comment{Initializing the best candidate to add}
\State bestDelay$=E(\mathcal P_e)$ \label{lst1:line:3}\Comment{Init best delay}
\For {$p\in \mathcal P \setminus \mathcal P_e$} \label{lst1:line:4}\Comment{For each peer not in the current \ed list}
	\If{$E(\mathcal P_e \cup\{ p\})\leq~$bestDelay$-\epsilon_\text{thr}$} \label{lst1:line:5} \Comment{If adding $p$ is good}%\Comment{Check if adding  $p$ improves the delay more than $\epsilon_\text{thr}$}
		\State $p_\text{best}^+=p$ \label{lst1:line:6}\Comment{Store the best candidate}
		\State bestDelay=$E(\mathcal P_e \cup p)$ \label{lst1:line:7}\Comment{Store the best delay}
	\EndIf	
\EndFor
\If {$p_\text{best}^+\neq -1$} \label{lst1:line:8} \Comment{If we found a best candidate}
     \State $\mathcal P_e\gets \mathcal P_e\cup \{p_\text{best}^+\}$ \label{lst1:line:9}\Comment{Update with the best candidate}
\EndIf
\State $p_\text{best}^-=-1$ \label{lst1:line:10}\Comment{Initializing the best candidate to remove}
\State bestDelay$=E(\mathcal P_e)$ \label{lst1:line:11}\Comment{Initializing the best delay}
\For {$p\in \mathcal P_e\setminus \{p_\text{best}^+\}$} \label{lst1:line:12} \Comment{Peer from $\mathcal P_e$ except $p_\text{best}^+$}
	\If {$E(\mathcal P_e\setminus \{p\})<~$bestDelay$+\epsilon_\text{thr}$} \label{lst1:line:13}\Comment{If removing $p$ is good}%\Comment{Check if removing $p$ increases the delay less than $\epsilon_\text{thr}$}
		\State $p_\text{best}^-=p$ \label{lst1:line:14}\Comment{Store the best candidate}
		\State bestDelay$=E(\mathcal P_e\setminus \{p\})$ \label{lst1:line:15}\Comment{Store the best delay}
	\EndIf
\EndFor
\If {$p_\text{best}^-\neq -1$} \label{lst1:line:16} \Comment{Check if found a best candidate}
     \State $\mathcal P_e\gets \mathcal P_e\setminus \{p_\text{best}^-\}$ \label{lst1:line:17}\Comment{Update with the best candidate}
\EndIf
\State \Return $\mathcal P_e$ \label{lst1:line:18}\Comment{Return the \ed set}
\EndProcedure

\end{algorithmic}
\caption{Pseudocode of the {\tt AveMinDelay(AMD} variant of {\tt SelectEndorsers} }\label{alg:opt_endorse1}
\end{figure}





% \subsubsection{SelectEndorsers-SingleAverage}

% Similar to the \texttt{SelectEndorsers-AveMinDelay(AMD}, the \texttt{SelectSingleAverage} returns a set of endorser peers as output, but, it does not receive $\epsilon$ as the input parameter. Differently from the \texttt{SelectEndorsers-AveMinDelay(AMD}, the \texttt{SelectSingleAverage} relies on an internal threshold delay called $d_t$ which is calculated by using the average of all the \en latency samples of the client~(line \ref{lst2:line:2}). 


% The score of each peer is defined as the probability of having the \en latencys of that peer before $d_t$, which is calculated by using the cumulative density function of the \en latencys of that peer until the $d_t$, and the peers with the score more than or equal to \texttt{}{MYSTERY METRIC} will be selected as the endorser peers~(line \ref{lst2:line:4}) and will be returned to the \texttt{Optimizer} algorithm~(line \ref{lst2:line:5}). The pseudocode of  \texttt{SelectSingleAverage} is provided in Fig.~\ref{alg:opt_endorse2}.

% \paolo{Must explain why we use the median (i.e., 1/2) and not the average.}  


% \begin{figure}[!tb]
% \scriptsize
% %\renewcommand\figurename{Listing}
% \label{alg:opt_endorse2}
% \begin{algorithmic}[1]
% \renewcommand{\algorithmicrequire}{ Input:}}
% \renewcommand{\algorithmicensure}{ Output:}}
% \Require $P$: Set of \ed peers 
% \Require $P_e$: Candidate list of \ed peers 
% \Require $\mathcal X=\{X_p\}_{p\in P}$: Endorsement delays for all the peers with their empirical distributions
% \Procedure{SelectEndorsers-SIngleAverage}{$P,P_e,\mathcal X$}
%     \State $d_{t} \gets E_{p\in P}(X_p)$ \label{lst2:line:2}\Comment{Delay threshold is the average delay for the peers $\in P$}
%     \State MisPar $\gets$ ???? \label{lst2:line:3}\Comment{MISTERY PARAMETER}
%     \State $P_e \gets \{p \in P: F_{X_p}(d_t) \geq$ MisPar\}\label{lst2:line:4}\Comment{The $P_e$ set contains the current best peers}
%     \State \Return $P_e$\label{lst2:line:5}\Comment{Return endorsement set}
% \EndProcedure

% \end{algorithmic}
% \caption{Pseudocode of the second variant of {\tt SelectEndorsers} }\label{alg:opt_endorse2}
% \end{figure}


\subsubsection{ApproxLastTwoDelays(ALTD)}


The \texttt{ApproxLastTwoDelays(ALTD)} procedure receives as inputs the set of all endorsers, the set of previous endorsers, the sequence number of the transaction, the past history of response delays, and the modified version of the response delays for the last two recent transactions. It returns a set of selected peers as the new endorsers.

In summary, each client can use the response delays $X^{(n-1)}$ and $X^{(n-2)}$ to select the best endorser peers for the current transaction $n$. The response delays in $X^{(n-1)}$ can be used to select the least loaded peers, as these delays carry the most recent information about the peer's queuing state. Also, by comparing the delays in $X^{(n-1)}$ with the ones in $X^{(n-2)}$, it is possible to estimate if the load on the peers has increased or not. The challenge is that the delays for some peers are undefined, either because the corresponding response has not arrived yet or no endorsement request was sent. So, this algorithm will use the approximated response delays $Y^{(1)}$ and $Y^{(2)}$ which is derived from $X^{(n-1)}$ and $X^{(n-2)}$ to overcome this problem.
The number of endorsers is denoted by $R$ and it is initialized to $Q$. At each transaction, we allow $R$ to vary by at most one peer. We set $\epsilon_\text{est} =1~ns$ a threshold value much smaller than all the delays involved in the endorsement process~(line \ref{lst2:line:2}). If still, no delay responses are available for the previous transaction, it will keep the previous approximated delays as the new response delays and will choose half of the peers as the number of new endorsers~(lines \ref{lst2:line:3} to \ref{lst2:line:41}). Otherwise, \texttt{ApproxLastTwoDelays(ALTD)} generates a set $\mathcal A$ of non-zero values of $X^{(n-1)}$~(lines \ref{lst2:line:5} and \ref{lst2:line:6}). For each peer $p$ belonged to the set $\mathcal P_e$, if the last response delay is not received yet, it is reasonable to consider that this value will be greater than the maximum value of the received responses for this transaction, So, it will be replaced in the $Y^{(1)}$ with the maximum value of $(\mathcal A)$ increased by the $\epsilon_\text{est}$. Otherwise, if the response delay is available, it will use the available response delays~(lines \ref{lst2:line:7} to \ref{lst2:line:11}). 
As we did not send to the rest of the peers that were not in the previous set of selected endorsers, we propose to keep their delay responses of the $Y^{(2)}$ for the $Y^{(1)}$ as well~(lines \ref{lst2:line:12} to \ref{lst2:line:13}). If all the responses are not received we decrease the number of endorsers by one, otherwise, it greedily increases the number of endorsers by one~(lines \ref{lst2:line:131} to \ref{lst2:line:134}).
Now, comparing the sum of approximated response delays in $Y^{(1)}$ with the $Y^{(2)}$ will let the \texttt{ApproxLastTwoDelays(ALTD)} to decide over decreasing or increasing the number of endorsers by assigning the new value to $R$~(lines \ref{lst2:line:14} to \ref{lst2:line:17}). It is possible to select $R$ peers with the least delay value among $Y^{(1)}$ and assign those peers to the set $\mathcal P_e$~(line \ref{lst2:line:18}). The algorithm then prepares the $Y^{(2)}$ for the next transaction by copying the values in $Y^{(1)}$ to $Y^{(2)}$ and returns the $\mathcal P_e$~(lines \ref{lst2:line:19} to \ref{lst2:line:20}). The pseudocode of \texttt{ApproxLastTwoDelays(ALTD)} is provided in Fig.~\ref{alg:opt_endorse2}.


\begin{figure}[!tb]
\scriptsize
\label{alg:opt_endorse2}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{ Input:}
\renewcommand{\algorithmicensure}{ Output:}
\Require $\mathcal P$: Set of \ed peers 
\Require $\mathcal P_e$: Candidate list of \ed peers 
\Require $n$: Transaction sequence number 
\Require $\mathcal X=\{X^{(k)}\}_{k=1,\ldots,n}$: Past history of response delays
\Require $\mathcal Y=\{Y^{(k)}\}_{k=1,2}$ : Approximated $X^{(n)}$ for two recent transactions

% \Procedure{ApproxLastTwoDelays(ALTD)}{$\mathcal P,\mathcal P_e,n,\mathcal X,\mathcal Y$}\label{lst2:line:1}
\Procedure{SelectEndorsers-ALTD}{$\mathcal P,\mathcal P_e,n,\mathcal X,\mathcal Y$}\label{lst2:line:1}
 \State $\epsilon_\text{est} \gets 1$~ns\label{lst2:line:2}\Comment{Set an enough small delay threshold}
\If{$\max(X^{(n-1)})=0$}\label{lst2:line:3}\Comment{If no $\text{X}^{(n-1)}$ is received}
  \State $Y^{(1)} \gets Y^{(2)}$ \label{lst2:line:4}\Comment{Use approx. delays of $\text{TX}^{(n-2)}$ for $\text{TX}^{(n-1)}$}
  \State $R\gets |\mathcal P|/2$\label{lst2:line:41}\Comment{Selects half of the peers based on~\eqref{eq:r1}}
\Else\label{lst2:line:5}\Comment{We received at least one response}
    \State $\mathcal A \gets \emptyset$\label{lst2:line:50}
    \For{$p\in \mathcal P_e$}\label{lst2:line:51}
       \If{$X^{(n-1)}_p \neq 0$}\label{lst2:line:52}\Comment{If there is a response from peer $p$}
         \State $\mathcal A \gets \mathcal A \cup \{X^{(n-1)}_p\}$\label{lst2:line:6}\Comment{Add it to the set $\mathcal A$} %\Comment{Update the set of available response delays for $\text{TX}^{(n-1)}$}
       \EndIf
     \EndFor
   \For {$p \in \mathcal P_e$}\label{lst2:line:7}
    \If {$X^{(n-1)}_p = 0$}\label{lst2:line:8}\Comment{No response from $p$ for $\text{TX}^{(n-1)}$}
      \State $Y^{(1)}_p = \max\{\mathcal A\}+\epsilon_\text{est} $ \label{lst2:line:9}\Comment{Approximate the missing delay}
    \Else \label{lst2:line:10}
      \State $Y^{(1)}_p = X^{(n-1)}_p$ \label{lst2:line:11}\Comment{Use the available response delay}
    \EndIf
  \EndFor
  \For {$p \notin \mathcal P_e$}\label{lst2:line:12}\Comment{For non-endorser peers in $\text{TX}^{(n-1)}$}
    \State $Y^{(1)}_p = Y^{(2)}_p$ \label{lst2:line:13}\Comment{Use approx. values from $\text{TX}^{(n-2)}$}
  \EndFor
  \If{$|\mathcal A| < |\mathcal P_e| $}\label{lst2:line:131}\Comment{If some responses are not received yet}
    \State $R\gets \max\{|\mathcal P_e|-1,1\}$\label{lst2:line:132}\Comment{Decrease the number of endorsers}
  \Else\label{lst2:line:133}
    \State $R\gets \min\{|\mathcal P_e|+1,|\mathcal P|\}$\label{lst2:line:134}\Comment{Increase the number of endorsers} 
  \EndIf
\EndIf
\If{$\sum_p Y^{(1)}_p < \sum_p Y^{(2)}_p $}\label{lst2:line:14}\Comment{If congestion seems to decrease}
  \State $R\gets \min\{R+1,|\mathcal P|\}$\label{lst2:line:15}\Comment{Increase the number of endorsers} 
\Else\label{lst2:line:16}
  \State $R\gets \max\{R-1,1\}$\label{lst2:line:17}\Comment{Decrease the number of endorsers}
\EndIf
\State $\mathcal P_e \gets$ \texttt{ Select-peers-with-min-delay}($R$,$Y^{(1)}$)\label{lst2:line:18}\Comment{Best $R$}
\State $Y^{(2)} \gets Y^{(1)} $\label{lst2:line:19} \Comment{Shifting the $Y^{(1)}$ values to $Y^{(2)}$}
\State \Return $\mathcal P_e$ \label{lst2:line:20}\Comment{Return the \ed set}
\EndProcedure
\end{algorithmic}
\caption{Pseudocode of the {\tt ApproxLastTwoDelays} variant of {\tt SelectEndorsers} }\label{alg:opt_endorse2}
\end{figure}



\subsubsection{ApproxLastOneDelay(ALOD)}

The \texttt{ApproxLastOneDelay(ALOD)} receives a set of \ed peers $P$, the transaction sequence number $n$, the \en response delays for all the peers $\mathcal X$, and the modified version of the response delays for last transactions $\mathcal Y$ as input and returns a set of \ed peers $\mathcal P_e$ as output. 
The \texttt{ApproxLastOneDelay(ALOD)} can be considered as a simplified version of the \texttt{SelectApproxLastTwoDelays}, it is not deciding over the number of endorser peers $R$ for each transaction based on the total load change. Instead, based on the \texttt{Subversion} provided to it, it will select $k$ peers with minimum response delays for the last transaction. Similarly to \texttt{ApproxLastTwoDelays(ALTD)}, it sets $\epsilon_\text{est} =1~ns$~(line \ref{lst31:line:2}). If still no delay responses are available for previous transaction, it will keep the previous approximated delays as the new response delays, then it prefers the non-endorser peers of previous transaction by setting their response delays to zero~(lines \ref{lst31:line:3} to \ref{lst31:line:4}). Otherwise, it generates a set $\mathcal A$ of available(i.e., non-zero) response delays referred to $\text{TX}^{(n-1)}$ from each peer of the previous endorsers set $\mathcal P_e$~(lines \ref{lst31:line:5} to \ref{lst31:line:6}). 

For each peer $p$ belonged to the set $\mathcal P_e$, if the last response delay is not received yet, it will be replaced in the $Y^{(1)}$ with the maximum value in $(\mathcal A)$ increased by the $\epsilon_\text{est}$. Otherwise, if the response delay is available, it will use the available response delays~(lines \ref{lst31:line:7} to \ref{lst31:line:11}). Also, it keeps the delay responses of the $Y^{(2)}$ for the $Y^{(1)}$ for the peers that were not part of $\mathcal P_e$~(lines \ref{lst31:line:12} to \ref{lst31:line:13}). Now, the  \texttt{SelectPeersAndDelays} procedure takes \texttt{SubVersion}, $Y^{(1)}$, and $\mathcal P$ as input and will return as output $k$ and $Y^{'(1)}$  which are the number of endorser peers and the final modified response delays respectively~(line \ref{lst31:line:131}). Then, it  selects $k$ peers with the least delay value among $Y^{'(1)}$ and assign those peers to the set $\mathcal P_e$~(line \ref{lst31:line:14}). The algorithm then prepares the $Y^{(2)}$ for the next transaction by copying the values in $Y^{(1)}$ to $Y^{(2)}$ and returns the $\mathcal P_e$~(lines \ref{lst31:line:15} to \ref{lst31:line:16}). The pseudocode of \texttt{ApproxLastOneDelay(ALOD)} is provided in Fig.~\ref{alg:opt_endorse3}.


\begin{figure}[!tb]
\scriptsize
\label{alg:opt_endorse3}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{ Input:}
\renewcommand{\algorithmicensure}{ Output:}
\Require $\mathcal P$: Set of \ed peers 
\Require $n$: Transaction sequence number 
\Require $\mathcal X=\{X_p\}_{p\in P}$: Response delays for all the peers with their empirical distributions
\Require $\mathcal Y=\{Y^{(k)}\}_{k=1,2}$ : Approximated $X^{(n)}$ for two recent transactions
\Procedure{SelectEndorsers-ALOD}{$\mathcal P,\mathcal X,\mathcal Y$}
  \State $\epsilon_\text{est} \gets 1$~ns\label{lst31:line:2}\Comment{Set an enough small delay threshold.}
  \If{$\max(X^{(n-1)})=0$}\label{lst31:line:3}\Comment{If no $\text{X}^{(n-1)}$ is received}
    \State $Y^{(1)} \gets Y^{(2)}$ \label{lst31:line:31}\Comment{Use approx. delays of $\text{TX}^{(n-2)}$ for $\text{TX}^{(n-1)}$}
    \For {$p \notin \mathcal P_e$}\label{lst31:line:32}
      \State $Y^{(1)}_p = 0$ \label{lst31:line:4}\Comment{Preferring the previous Non-endorser peers}
    \EndFor
  \Else \label{lst31:line:5}
    \State $\mathcal A \gets \emptyset$\label{lst31:line:50}
    \For{$p\in \mathcal P_e$}\label{lst31:line:51}
       \If{$X^{(n-1)}_p \neq 0$}\label{lst31:line:52}\Comment{If there is a response from peer $p$}
         \State $\mathcal A \gets \mathcal A \cup \{X^{(n-1)}_p\}$\label{lst31:line:6}\Comment{Add it to the set $\mathcal A$}
       \EndIf
     \EndFor
%    \State $\mathcal A \gets \{X^{(n-1)}_p\}_{p\in \mathcal P_e, X^{(n-1)}_p \neq 0}$ \label{lst31:line:6}\Comment{Set of available response delays for $\text{TX}^{(n-1)}$}
   \For {$p \in \mathcal P_e$}\label{lst31:line:7}
    \If {$X^{(n-1)}_p = 0$}\label{lst31:line:8}
      \State $Y^{(1)}_p = \max\{\mathcal A\}+\epsilon_\text{est} $ \label{lst31:line:9}\Comment{Approximate the missing delay}
    \Else \label{lst31:line:10}
      \State $Y^{(1)}_p = X^{(n-1)}_p$ \label{lst31:line:11}\Comment{Use the available response delay}
    \EndIf
   \EndFor
   \For {$p \notin \mathcal P_e$}\label{lst31:line:12}
    \State $Y^{(1)}_p = X^{(n-2)}_p$ \label{lst31:line:13}\Comment{Use previous response delays}
   \EndFor
  \EndIf
  \State $k,Y^{'(1)} \gets$ {\tt SelectPeersAndDelays}(\texttt{SubVersion},$Y^{(1)}$,$\mathcal P$) \label{lst31:line:131}%\Comment{Returns the response delays and number of peers based on \texttt{SubVersion}}
  \State $\mathcal P_e \gets$ \texttt{ Select-peers-with-min-delay}($k$,$Y^{'(1)}$)\label{lst31:line:14}\Comment{Best $k$}
  \State $Y^{(2)} \gets Y^{(1)} $\label{lst31:line:15} \Comment{Shifting the $Y^{(1)}$ values to $Y^{(2)}$}
  \State \Return $\mathcal P_e$\label{lst31:line:16}\Comment{Return endorsement set}
\EndProcedure

\end{algorithmic}
\caption{Pseudocode of the {\tt ApproxLastOneDelay} variant of {\tt SelectEndorsers} }\label{alg:opt_endorse3}
\end{figure}


\paragraph{SelectPeersAndDelays-SubVersions}

We propose three \texttt{SubVersion}s, \texttt{SubVersion=1} with approximation of~\eqref{eq:r1} sets $k=|Q/2|$ or selects half of the peers and returns $k$ and the same vector of modified response delays $Y^{(1)}$~(lines \ref{lst31:line:2} and \ref{lst31:line:3}), while the two remaining ones can be considered as the economic  \texttt{SubVersion}s of the \texttt{ApproxLastOneDelay(ALOD)} in terms of network resource consumption as they set $k=1$ as the number of endorser peers. \texttt{SubVersion=2} returns $k=1$ and the same vector of modified response delays $Y^{(1)}$~(lines \ref{lst31:line:4} and \ref{lst31:line:5}), while inspired from~\cite{end12}, \texttt{SubVersion=3} selects randomly half of the $Y^{(1)}$~(lines \ref{lst31:line:6} and \ref{lst311:line:7}) to be considered in the best peers selection. It returns $k=1$ and a modified vector of the $Y^{(1)}$ as $Z^{(1)}$ which has replaced with \texttt{infinite} the response delays that are not part of the reandomly selected peers~(lines \ref{lst31:line:8} to \ref{lst31:line:12}). This randomeness will avoid to overload the best peer in case of multiple clients. The pseudocode of {\tt SelectPeersAndDelays} is provided in Fig.~\ref{alg:opt_endorse31}.


%This can be done by replacing line \ref{lst31:line:14} of Fig.~\ref{alg:opt_endorse31} with line \ref{lst31:line:1} or lines \ref{lst31:line:2} to \ref{lst31:line:3} of Fig.~\ref{alg:opt_endorse31} respectively. 

%Using the same algorithm offered in \texttt{ApproxLastOneDelay(ALOD)}, we proposed two economic sub-version of the \texttt{ApproxLastOneDelay} in terms of network resource consumption by: 1) considering only one best peer with the least response delay among $Y^{(1)}$ as the only endorser peer~(line \ref{lst31:line:1} of Fig), Or 2) inspired from~\cite{end12}, selecting randomly half of the $Y^{(1)}$ instead of all the peers, and choosing the peer with the least response delay among them as the only endorser peer. This can be done by replacing line \ref{lst31:line:14} of Fig.~\ref{alg:opt_endorse31} with line \ref{lst31:line:1} or lines \ref{lst31:line:2} to \ref{lst31:line:3} of Fig.~\ref{alg:opt_endorse31} respectively. 

\begin{figure}[!tb]
\scriptsize
\label{alg:opt_endorse31}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{ Input:}
\renewcommand{\algorithmicensure}{ Output:}
\Require $\mathcal P$: Set of \ed peers 
\Require $\texttt{SubVersion}$: SubVersion of the \texttt{ApproxLastOneDelay} 
\Require $Y^{(1)}$ : Modified version of the response delays for the last transaction
\Procedure{SelectPeersDelays}{$\texttt{SubVersion},\mathcal P,Y^{(1)}$}\label{lst31:line:1}
  \If{$\texttt{SubVersion}=1$}\label{lst31:line:2}\Comment{Basic version}
    \State \Return $|\mathcal P|/2,Y^{(1)}$\label{lst31:line:3}\Comment{Half of the peers and all the response delays}
  \EndIf
  \If{$\texttt{SubVersion}=2$}\label{lst31:line:4}
    \State \Return $1,Y^{(1)}$\label{lst31:line:5}\Comment{One of the peers and all the response delays}
  \EndIf
  \If{$\texttt{SubVersion}=3$}\label{lst31:line:6}
    \State $\mathcal P^{'} \gets$ \texttt{ Select-randomly}($|\mathcal P|/2$,$\mathcal P$) \label{lst31:line:7}\Comment{Random half of the $\mathcal P$}
     \State $Z^{(1)} \gets Y^{(1)}$ \label{lst31:line:8}\Comment{Temporary place for response delays}
     \For {$p \in \mathcal P$}\label{lst31:line:9}
      \If {$p \notin \mathcal P^{'}$}\label{lst31:line:10}
        \State $Z^{(1)}_p = \text{infinite} $ \label{lst31:line:11}\Comment{Removing the chance for peer $p$}
      \EndIf
    \EndFor
    \State \Return $1,Z^{(1)}$\label{lst31:line:12}\Comment{One of the peers and all the response delays}
  \EndIf
\EndProcedure

\end{algorithmic}
\caption{Pseudocode of the {\tt SelectPeersDelays} variants of {\tt ApproxLastOneDelay} }\label{alg:opt_endorse31}
\end{figure}



 
\subsubsection{OracleOptimalDelays(OOD)}

As a reference for all the \en algorithms, we define an online optimal endorsement peer selection policy that minimizes the response delay, given a fixed number of $R$ \en peers.
We assume to have an oracle knowing, in advance, the response delay of any \en request if sent to a specific peer. Thus, we assume that the oracle knows, for any peer $p$, (i) the time $T^\text{busy}_p$ at which the peer will finish (or has finished) to serve the last received \en request, (ii) the processing time $\tau_p^\text{proc}$ of the \en request and (iii) the overall network delay $\tau^\text{net}_p$ between each client and the peer~(line \ref{lst4:line:1}). Thus, at the current time $t^\text{now}$, the response will be received from peer $p$ at a virtual time $T^\text{resp}_p$~(lines \ref{lst4:line:2} and  \ref{lst4:line:3}), computed as follows:

\begin{equation}\label{eq:oracle}
T^\text{resp}_p=\max\{t^\text{now},T^\text{busy}_p \}+\tau_p^\text{proc}+\tau^\text{net}_p
\end{equation}

%\paolo{The notation has been chosen without checking if already defined. If yes, please revise it according to the pre-existing notation}

Now the oracle will choose $R$ \en peers based on the virtual times:
\begin{itemize}
\item one \en request will be sent to the peer with the smallest virtual time since this will minimize the response delay~(line \ref{lst4:line:4});
%\item when $R>1$, the second \en request will be sent to the peer with the largest virtual time, since this will load the ``slowest'' peer with a useless request;
\item the remaining $R-1$ \en requests (if any) will be sent to the peers in decreasing order to virtual time since this will allow loading the ``slowest'' peers with requests whose responses will be received too late and will reduce the load on the ``fastest" peers, for the sake of future \en requests~(lines \ref{lst4:line:9} to \ref{lst4:line:18}).
It is trivial that, The oracle can ultimately minimize the response delay at each endorsement process, by sending the request just to the peer with the smallest virtual time among $R$ peers and not sending to other peers by setting $R=1$. This will avoid overloading other peers with useless requests that lead to having a system with the perfect load.

\end{itemize}
The pseudocode of {\tt OracleOptimalDelays} is provided in Fig.~\ref{alg:opt_endorse4}.

 \begin{figure}[!tb]
 \scriptsize
 \label{alg:lastdelay}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{ Input:}
 \renewcommand{\algorithmicensure}{ Output:}
 \Require $\mathcal P$: Set of \ed peers 
 \Require $R$: Number of \ed peers 
 \Require $T^\text{busy}$: Vector of finishing time for all the endorser peers 
 \Require $\tau^\text{net}$: Vector of the network delay between the client and the peers in $\mathcal P$
 \Require $\tau^\text{proc}$: Vector of the current endorsement processing time for peers in $\mathcal P$
 \Procedure{SelectEndorsers-OOD}{$\mathcal P,R,T^\text{busy},\tau^\text{net},\tau^\text{proc}$} \label{lst4:line:1}
 \For {$p \in \mathcal P$}\label{lst4:line:2}\Comment{For each peer according to \ref{eq:oracle}}
   \State $T^\text{resp}_p \gets \max(t^\text{now},T^\text{busy}_p)+\tau_p^\text{proc}+\tau^\text{net}_p$ \label{lst4:line:3}\Comment{Update virtual time}
 \EndFor
 \State $\mathcal P_e \gets$ \texttt{ Peer-with-min-virtual-response-time}($T^\text{resp}$) \label{lst4:line:4}%\Comment{Selecting the best peer with min virtual time}
 \State $\mathcal P^{'} \gets \mathcal P \setminus \mathcal P_e$  \label{lst4:line:5}\Comment{Temporary set of peers except the best peer}
 \For {$p \in \mathcal P_e$}
   \State $T^\text{busy}_p \gets  \min(T^\text{resp})$ \label{lst4:line:7}\Comment{Update the {\tt busy} time for the best peer}
 \EndFor
%  \If{$\text{OptimalOracle} = \text{true}$} \label{lst4:line:8}\Comment{If it is the {\tt OptimalOracle}}
    \State $R \gets R-1$ \label{lst4:line:9}
    \While{$R > 0$}{ \label{lst4:line:10}\Comment{If still there is endorsement request}
       \For {$p \in \mathcal P'$}\label{lst4:line:11}
          \If{$T^\text{resp}_p = \text{max}(T^\text{resp})$} \label{lst4:line:12}\Comment{Select the worst virtual time}
             \State $\mathcal P_e \gets \mathcal P_e \cup \{p\}$\label{lst4:line:13}\Comment{Adding the new worst peer}
             \State $T^\text{busy}_p \gets  T^\text{resp}_p$\label{lst4:line:14}\Comment{Updating the peer {\tt busy} time} 
             \State $T^\text{resp}_p \gets 0$\label{lst4:line:15}\Comment{Remove the current worst response time} 
             \State $\mathcal P^{'} \gets \mathcal P^{'} \setminus  \{p\}$\label{lst4:line:16}\Comment{Remove the selected peer } 
             \State $R \gets R-1$ \label{lst4:line:17}\Comment{Reduce the remained requests} 
        \EndIf
     \EndFor}
  \EndWhile
% \EndIf
\State \Return $\mathcal P_e$\label{lst4:line:18}\Comment{Return endorsement set}

\EndProcedure
 \end{algorithmic}
 \caption{Pseudocode of the {\tt OracleOptimalDelays} variant of {\tt SelectEndorsers} }\label{alg:opt_endorse4}
 \end{figure}


% \subsubsection{SuperOracleOptimalDelays(SOOD)}


% In theory, similar to the oracle defined in the previous section, it is possible to have a super-oracle that according to~\eqref{eq:oracle} knows in advance the response delay of any endorsement request if it is sent to a specific peer. This super-oracle can ultimately minimize the response delay at each endorsement process, by sending the request just to the peer with the smallest virtual time among $R$ peers and not sending to other peers~(lines \ref{lst4:line:1} to~\ref{lst4:line:7} of Fig.~\ref{alg:opt_endorse4}). This will avoid overloading other peers with useless requests that lead to having a system with the perfect load.



\paolo{Add comments for each graph. Do not repeat the numerical results (the reader is able to see the numbers) but discuss what we learn from each graph.}

\subsection{Simulations results}

To evaluate the performance of the different variants of the proposed algorithm using omnet++, we built a network similar to Fig.~\ref{figure:QueuingModel} including one client and eight servers with an average service time of 1[s] as the endorser peers. We performed the simulations considering 2 cases:
\begin{itemize}
\item network delays are negligible with respect to the service times of the servers, 
\item network delays are comparable or dominant with respect to the service times of the servers.
\end{itemize}
In the first case, the delays between the client and the servers are considered zero while for the second case, the delays between the client and the servers are started from zero for the first server and increased by one second for each next server such that the last server has a delay of seven seconds. For both cases the total load is controlled by changing the factor $\gamma$ based on~\eqref{eq:7} and ~\eqref{eq:lambda}. 
The simulation results are shown in Fig.~\ref{figure:variants_zeroDelay1} and Fig.~\ref{figure:variants_linearDelay1}.


As expected, the {\tt OracleOptimalDelays(OOD)} with $R=1$ has the best results with the lowest experienced response delays. 
% The superiority of the {\tt SuperOracleOptimalDelays(SOOD)} over the {\tt OracleOptimalDelays(OOD)} is due to theoreticaly perfect awareness of the system and thus sending only to the best server while the other needs to send to all of them.
The \texttt{AveMinDelay(AMD} behaviour is completely dependent on selecting a proper delay thresholds(i.e. $\epsilon_\text{thr}$) with respect to the dominant delay generators in the model(i.e. path delay, processing delay, etc.) and the distance between two $\epsilon_\text{thr}$. We chose $\epsilon_\text{thr}=$ 0.05[s] and 0.01[1] which is negligible with respect to the above-mentioned delays. The results are not promising in the case of zero delays in the paths where it is affected by the randomness of the processing time which is the dominant delay generator. 

\begin{figure}[!tb]
    \centering
    \includegraphics[width=8cm]{Figures/Q8C1MM1d0_Dly-Gamma(10-90).pdf}
    \caption{Simulation results for the algorithm variants ($\gamma \in [0.1,0.9]$)}
    \label{figure:variants_zeroDelay1}
\end{figure}

\begin{figure}[!tb]
    \centering
    \includegraphics[width=8cm]{Figures/Q8C1MM1d0_Dly-Gamma(10-90)Linear.pdf}
    \caption{Simulation results for the algorithm variants ($\gamma \in [0.1,0.9]$)}
    \label{figure:variants_linearDelay1}
\end{figure}

\begin{figure}[!tb]
    \centering
    \includegraphics[width=8cm]{Figures/Q8C1MM1d0_Dly-Gamma(10-90)2.pdf}
    \caption{Simulation results for the algorithm variants ($\gamma \in [0.1,0.9]$)}
    \label{figure:variants_zeroDelay1}
\end{figure}

\clearpage
% Fig.~\ref{figure:variants_zeroDelay2},
%Fig.~\ref{figure:variants_zeroDelay3}, Fig.~\ref{figure:variants_linearDelay1} and
% , Fig.~\ref{figure:variants_linearDelay2} and
%Fig.~\ref{figure:variants_linearDelay3}.



% \begin{figure}[!tb]
%     \centering
%     \includegraphics[width=8cm]{Figures/Q8C1MM1d0_Dly-Gamma(100-700).pdf}
%     \caption{Simulation results for the algorithm variants ($\gamma \in [1,7]$)}
%     \label{figure:variants_zeroDelay2}
% \end{figure}

% \begin{figure}[!tb]
%     \centering
%     \includegraphics[width=8cm]{Figures/Q8C1MM1d0_Dly-Gamma(10-700).pdf}
%     \caption{Simulation results for the algorithm variants ($\gamma \in [0.1,7]$)}
%     \label{figure:variants_zeroDelay3}
% \end{figure}




% \begin{figure}[!tb]
%     \centering
%     \includegraphics[width=8cm]{Figures/Q8C1MM1d0_Dly-Gamma(100-700)Linear.pdf}
%     \caption{Simulation results for the algorithm variants ($\gamma \in [1,7]$)}
%     \label{figure:variants_linearDelay2}
% \end{figure}

% \begin{figure}[!tb]
%     \centering
%     \includegraphics[width=8cm]{Figures/Q8C1MM1d0_Dly-Gamma(10-700)Linear.pdf}
%     \caption{Simulation results for the algorithm variants ($\gamma \in [0.1,7]$)}
%     \label{figure:variants_linearDelay3}
% \end{figure}


\begin{figure}[!tb]
    \centering
    \includegraphics[width=8cm]{Figures/Q8C1MM1d0_Dly-Gamma10-Cv(0-5).pdf}
    \caption{Coefficient of variation for the algorithms for $\gamma =0.1$}
    \label{figure:Cv1}
\end{figure}



\begin{figure}[!tb]
    \centering
    \includegraphics[width=8cm]{Figures/Q8C1MM1d0_Dly-Gamma70-Cv(0-5).pdf}
    \caption{Coefficient of variation for the algorithms for $\gamma =0.7$}
    \label{figure:Cv7}
\end{figure}

% \begin{figure}[!tb]
%     \centering
%     \includegraphics[width=8cm]{Figures/Q8C1MM1d1_Dly-Gamma70-Cv(0-5).pdf}
%     \caption{Coefficient of variation for the algorithms for $\gamma =0.7$}
%     \label{figure:Cv1}
% \end{figure}






















\clearpage
\begin{figure}[!tb]
\scriptsize
\label{alg:lastdelay}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{ Input:}
\renewcommand{\algorithmicensure}{ Output:}
\Require $\mathcal P$: Set of \ed peers 
\Require $\mathcal P_e$: Past set of \ed peers
\Require $\epsilon_\text{h} $: Hysteresis threshold for the delay
\Procedure{UpdateDelay}{endorsment}
\State $p=$peer(endorsment) %\Comment{Response time}
\State $d=$response-delay(endorsment)%\Comment{Response time}
\State $X^\text{old}_p=X^\text{new}_p$
\State $X^\text{new}_p=d$
\EndProcedure

\Procedure{SelectEndorsers-DeltaDelay}{$\mathcal P,\mathcal P_e$}
%   \State $R=|\mathcal P_e|$ 
  \If {$\sum_p X^\text{old}_p\leq\sum_p X^\text{new}_p$} \Comment{Check the congestion}
%   	\State $R=\max\{|\mathcal P_e|-1,1\}$\Comment{More congestion, thus reduce $R$}
%   	\State $R=\max\{R-1,1\}$\Comment{More congestion, thus reduce $R$}
  	\State $R=\max\{|\mathcal P_e|-1,1\}$\Comment{More congestion, thus reduce $R$}
%%<<<<<<< CONFLICT
%%  	\State $R=\max\{R-1,1\}$\Comment{More congestion, thus reduce $R$}
%%  \Else
%%%   	\State $R=\min\{|\mathcal P_e|+1,|\mathcal P|\}$\Comment{Less congestion, thus increase $R$}
%%  	\State $R=\min\{R+1,|\mathcal P|\}$\Comment{Less congestion, thus increase $R$}
%%  \EndIf
%%   \State $\mathcal P_e \gets \{p \in \mathcal P$ : $X_\text{new}[p] \in \{R \text{ smallest delays of } X_\text{new}\}\}$\label{lst9:line:3}\Comment{Compute the endorsers set $\mathcal P_e$}
%%  \State \Return $\mathcal P_e$\label{lst9:line:3}\Comment{Return endorsement set}
%%\EndProcedure
%%=======
  \Else
%   	\State $R=\min\{|\mathcal P_e|+1,|\mathcal P|\}$\Comment{Less congestion, thus increase $R$}
  	\State $R=\min\{|\mathcal P_e|+1,|\mathcal P|\}$\Comment{Less congestion, thus increase $R$}
%   	\State $R=\min\{R+1,|\mathcal P|\}$\Comment{Less congestion, thus increase $R$}
  \EndIf
  \State $\mathcal P_e \gets$ \texttt{ Select-peers-with-min-delay}($R$,$X^\text{new}$)\label{lst9:line:3}\Comment{Compute the endorsers set $\mathcal P_e$}
%   \State $\mathcal P_e \gets \{p \in \mathcal P$ : $X^\text{new}_p \in \{R \text{ smallest delays of } X^\text{new}\}\}$\label{lst9:line:3}\Comment{Compute the endorsers set $\mathcal P_e$}
  \State \Return $\mathcal P_e$\label{lst9:line:3}\Comment{Return endorsement set}
\EndProcedure
%%%%%% >>>>>>> 87c5c0905a9b26cf97f6bebf6c813563deeaf98b

\Procedure{SelectEndorsers-DeltaDelayHysteresis}{$\mathcal P,\mathcal P_e,\epsilon$}
%   \State $R=|\mathcal P_e|$ 
  \If {$\sum_p X^\text{old}_p+\epsilon_\text{h} <\sum_p X^\text{new}_p$} \Comment{Check the congestion}
  	\State $R=\max\{|\mathcal P_e|-1,1\}$\Comment{More congestion, thus reduce $R$}
%   	\State $R=\max\{R-1,1\}$\Comment{More congestion, thus reduce $R$}
  \ElsIf {$\sum_p X^\text{old}_p-\epsilon_\text{h} >\sum_p X^\text{new}_p$}
  	\State $R=\min\{|\mathcal P_e|+1,|\mathcal P|\}$\Comment{Less congestion, thus increase $R$}
%   	\State $R=\min\{R+1,|\mathcal P|\}$\Comment{Less congestion, thus increase $R$}
 % \Else 
  %\State ciao
  \EndIf
  \State $\mathcal P_e \gets$ \texttt{ Select-peers-with-min-delay}($R$,$X^\text{new}$)\label{lst9:line:3}\Comment{Compute the endorsers set $\mathcal P_e$}
%   \State $\mathcal P_e \gets \{p \in \mathcal P$ : $X^\text{new}_p \in \{R \text{ smallest delays of } X^\text{new}\}\}$\label{lst9:line:3}\Comment{Compute the endorsers set $\mathcal P_e$}
  \State \Return $\mathcal P_e$\label{lst9:line:3}\Comment{Return endorsement set}
\EndProcedure

\end{algorithmic}
\caption{Pseudocode of the {\tt DeltaDelay} and {\tt DeltaDelayHysteresis} variant of {\tt SelectEndorsers} }\label{alg:lastdelay}
\end{figure}

